Realistic Adversarial Data Augmentation for MR Image Segmentation

Neural network-based approaches can achieve high accuracy in various medical image segmentation tasks. However, they generally require large labelled datasets for supervised learning. Acquiring and manually labelling a large medical dataset is expensive and sometimes impractical due to data sharing and privacy issues. In this work, we propose an adversarial data augmentation method for training neural networks for medical image segmentation. Instead of generating pixel-wise adversarial attacks, our model generates plausible and realistic signal corruptions, which models the intensity inhomogeneities caused by a common type of artefacts in MR imaging: bias field. The proposed method does not rely on generative networks, and can be used as a plug-in module for general segmentation networks in both supervised and semi-supervised learning. Using cardiac MR imaging we show that such an approach can improve the generalization ability and robustness of models as well as provide significant improvements in low-data scenarios.

==> 6_novelty_statement.tex <==
%% 300 char.
To the best of our knowledge, the proposed adversarial data augmentation method is the first that designs and constructs realistic adversarial attacks in medical imaging, with the aim of improving the generalization and robustness of MR segmentation networks. The proposed method has three main advantages: 1) high effectiveness to the lack of labelled data; 2) better segmentation robustness on unseen pathological cases; 3) lower computational cost compared to GAN-based methods.

==> algorithms/adv_bias.tex <==
\begin{minipage}{\columnwidth}
        \begin{algorithm}[H]
            \caption{Generating Adversarial Bias Field}
            \label{alg:bias}
        \begin{algorithmic}[1]
            \STATE {\bfseries Input:}  Sample mini-batch $\{\image^{(i)}\}_{i=1}^{B}$ {from the training dataset}, a segmentation network  $\classfier_{seg} (\cdot; \theta)$
            \STATE {\bfseries Requires:}
            Bias field magnitude~$\alpha$, number of control points $k \times k$, step size~$\xi$, number of gradient ascent steps $n$. 
              \STATE {\bfseries Output:} adversarial bias field: $\Phi_{\rm bias}$
              \STATE For each image $\image^{(i)}$, randomly initialize a smooth bias field with control points $\cpoints^{(i)}$ %sampled from $[\log{(1-\alpha)},\log{(1+\alpha)}]$%
            \FOR{ $j=0$ {\bfseries to} $n-1$}
            \STATE 
            % Update $\cpoints_{adv}$ via taking the gradient of the divergence loss $\Distance$ with respect to $\cpoints$ on each input data $x_i$:\\     
            $\cpoints' \leftarrow\nabla\cpoints{\Distance} [\classfier_{seg}(\image;\theta),\classfier_{seg}(\biasfunc;\theta)]$ \\
            $\cpoints\leftarrow \proj (\cpoints+\xi\cdot \cpoints'/\|{\cpoints'}\|_2)$\\
              Interpolating $\cpoints$ to obtain smooth bias fields $\;\Phi_{\rm{bias}}$\\
              Normalize and rescale $\;\Phi_{\rm{bias}}$ to $[1-\alpha,1+\alpha]$.
           \ENDFOR
        \end{algorithmic}
        \end{algorithm}
\end{minipage}


==> algorithms/adv_morph.tex <==
    \begin{minipage}{\columnwidth}
        \begin{algorithm}[H]
            \caption{Generating Adversarial Diffemorphic Deformation.}
            \label{alg2}
        \begin{algorithmic}[1]
         \STATE {\bfseries Input:}  Sample mini-batch $\{\image^{(i)}\}_{i=1}^{B}$ {from the training dataset}, a segmentation network  $\classfier_{seg}(\cdot; \theta)$
            \STATE {\bfseries Requires:} Gaussian kernel $K_{\rm v}$ ($\sigma= \sigma_1$) to smooth the velocity field,
            Gaussian kernel $K_{\rm d}$ $(\sigma=\sigma_2)$ to regularize the deformation, learning rate ~$lr$, gradient ascent steps $n$
            \STATE {\bfseries Output:} adversarial morphological transformation $\Phi_{\rm morph}$
            \STATE Randomly initialize dense velocity field $\velocity$ and compute the initial deformation $\Phi_{\rm{morph}}$
            \FOR{ $i=0$ {\bfseries to} $n$}
            \STATE Update $\velocity$ via simple gradient ascent algorithm, in order to maximize the divergence:\\     
            $\velocity' \leftarrow\Delta_\velocity{\Distance} [\Phi_{\rm morph}(\classfier_{seg}(\image;\theta)),\classfier_{seg}(\difffunc;\theta)]$ \\
             $\velocity \leftarrow \beta \proj(\velocity+\lr{\velocity'/\|{\velocity'}\|_2})$
           \STATE $\velocity \leftarrow {K}_{\rm v}\star \velocity $
           \STATE $\Phi_{\rm c} \leftarrow \Phi_{\rm morph} \circ {\rm exp}(\velocity)$
           \STATE $\Phi_{\rm diff} \leftarrow K_d \star \Phi_{\rm c}$
            % where  ${\rm exp}(\velocity_{\rm adv})$ is computed using $\textit{Scaling and Squaring.}
           \ENDFOR
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}
\input{algorithms/adv_morph}


==> figures/adversarial_training.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/images/adversarial_training.png}
    \caption{Adversarial training with bias field perturbation.\notsure{I have put this figure in the introduction as well, but due to page limit, I have to squeeze it, the resolution is not good, let me know if you have any suggestions...}}
    \label{fig:adversarial training}
\end{figure}

==> figures/varing_iteration.tex <==
\begin{figure}
    \centering
    \includegraphics{figures/images/result_iteration.png}
    \caption{Caption}
    \label{fig:varying_iteration}
\end{figure}

==> morph_part/morph.tex <==
%% old intro
In this work, we introduce two novel types of transformation for data augmentation in medical imaging: intensity inhomogeneity (bias field) transformation and morphological transformation, which augment the variations in terms of  image  appearances  and  underlying  anatomical  shapes,  respectively.  These two  transformations  correspond  to  meaningful  changes  in  real  world.  Specifically, the bias field perturbation amplifies intensity non-uniformity, simulating potential image artefacts introduced by improper image acquisitions and reconstructions in MR images, whereas the morphological transformations represent intra-subject anatomical changes, which can be caused by organ motion, growth,atrophy, and disease progression. 

\subsubsection{Morphological Transformation}
Let us first define a dense deformation model for morphological transformation, encoding displacement at each pixel along x and y directions ${ \Phi_{\rm{morph}}}: \pixel \rightarrow \transformedpixel$. Here, $\Phi_{\rm{morph}}$ is a smooth one-to-one mapping between each point in one image and its corresponding point in the deformed image. Given an input image $\image \in \Reals^{H \times W}$ and a deformation field $\Phi_{\rm{morph}} \in \Reals^{H\times W\times 2}$, the deformed image can be viewed as the output of the following function:
\begin{equation}{
\label{eq:morphological transformation}
   \image_{\rm{morph}}=\difffunc= \image \circ {\Phi_{\rm morph}} (\velocity),}
\end{equation} 
where $\circ$ denotes an image warping operation. In this formulation, we assume that the deformation is evolved by the underlying constant velocity field ($\velocity$) over time t at each point: $\frac{\partial{{\Phi_{\rm{morph}}}^{(t)}}{\pixel}}{\partial{t}}=\velocity\pixel$. When t=0, the deformation is a identity mapping ${\Phi_{\rm{morph}}}^{(0)}=\rm{Id}$ . The final deformation field is obtained by integrating the stationary velocity field $\velocity$ over $t=[0,1]$, using a fast approximation algorithm called \emph{scaling and squaring}. To encourage the resulting difffemorphic transformation is a smooth, differentiable, invertible (one-to-one) mappings between manifolds, we further apply a fluid-like regularization to the velocity field and a diffusion-like regularization to the deformation field, which is achieved by convolving the velocity and generated displacement fields with two Gaussian kernels, respectively.




\subsection{Adversarial Training with Morphological Attack}
\begin{equation}
\label{opt:morpho}
\begin{aligned}
& \underset{\theta}{\text{minimize}}
& & \ComposeDistance[\Phi_{\rm morph}(\classfier_{seg}(\image;\theta);\velocity^{\rm adv}),\classfier_{seg}(\advdifffunc;\theta)] \\
& {\text{where } \underset{\velocity}\argmax}
& & \ComposeDistance[\Phi_{\rm morph}(\classfier_{seg}(\image;\theta),\velocity),\classfier_{seg}(\difffunc;\theta)] \\
& \text{subject to}
& & {\|\velocity\|\leq\beta}
\end{aligned}
\end{equation}

\input{algorithms/adv_morph}


\begin{table}[!ht]
\centering
\caption{\textbf{Segmentation accuracy of the proposed method and state-of-the-art data augmentation strategies in low-data settings.} Reported values are average Dice scores  for the left ventricular myocardium segmentation over 20 test subjects. Results with highest scores are represented by bold font.}
\label{tab:low_shot_w.o_morph}
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Require unlabelled data} & \multicolumn{2}{c}{\#  Training subjects} \\ \cmidrule(l){3-4} 
 &  & 1 & 3 \\ \midrule
Plain & \xmark & 0.293 & 0.544 \\
Basic Aug & \xmark & 0.560 & 0.796 \\\midrule
Mixup\cite{Zhang_2018_ICLR_mixup} & \xmark & 0.575 & 0.801 \\ 
VAT\cite{Miyato_2018_PAMI_VAT}  & \xmark & 0.570 & 0.811 \\
% Random Bias & \xmark & 0.618 & 0.808 \\
Adv Morph & \xmark & 0.541 & 0.798\\
Adv Bias & \xmark &  0.650 & \textbf{0.826} \\
% Adv Bias\&Morph & \xmark & \textbf{0.716} & \textbf{0.825} \\% 
\midrule
cGANs\cite{Chaitanya_2019_IPMI} & \yesmark & 0.710 & 0.823 \\ \bottomrule
\end{tabular}
\end{table}



==> tables/cross_poplation.tex <==
\begin{table}[!htbp]
\parbox{.45\linewidth}{
\centering
\caption{\textbf{Segmentation performance of the proposed method and baseline methods across five different populations.}}
\label{tab:cross_population_v1}
\begin{threeparttable}
\begin{tabular}{@{}lcccccr@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Intra-domain} & \multicolumn{4}{c}{\textbf{Cross-population}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}AVG\\ (n=86)\end{tabular}}} \\ \cmidrule(lr){2-6}
 & {\ul NOR} & {\ul DCM} & {\ul HCM} & {\ul MINF} & {\ul ARV} &  \\ \midrule
Baseline & 0.911 & 0.831 & 0.871 & 0.805 & 0.843 & 0.841 \\ 
+Mixup\cite{Zhang_2018_ICLR_mixup} & 0.901 & 0.803 & 0.881 & 0.789 & 0.844 & 0.833 \\
+VAT\cite{Miyato_2018_PAMI_VAT} & 0.909 & 0.843 & \textbf{0.891} & 0.824 & 0.843 & 0.853 \\
+Adv Bias (Proposed) & \textbf{0.912} & \textbf{0.871} & 0.890 & \textbf{0.847} & \textbf{0.853} & \textbf{0.868} \\ \midrule
% icolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  \\ \bottomrule
\end{tabular}
% \begin{tablenotes}
% \item Reported values are average Dice scoresfor the left ventricular myocardium segmentation evaluated on five different populations. Results with highest scores are represented by bold font.
% \end{tablenotes}
\end{threeparttable}
}
\end{table}



==> tables/low_shot.tex <==
\begin{table}[!htbp]
\parbox{.45\linewidth}{
\centering
 \caption{\textbf{Segmentation accuracy of the proposed method and state-of-the-art data augmentation strategies in both supervised (SU) and semi-supervised (SE) settings.} Reported values are average Dice scores for the left ventricular myocardium segmentation under 20 test subjects.} %Results with highest scores in each category are represented by bold font. }
\label{tab:low_shot_v1}
\begin{threeparttable}
\begin{tabular}{@{}cccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Setting} & \multicolumn{2}{c}{\#  labelled subjects for training} \\ \cmidrule(l){3-4} 
 &  & 1 & 3 \\ \midrule
% Plain & {SU} & 0.293 & 0.544 \\
Baseline & {SU} & 0.560 & 0.796 \\
+Mixup\cite{Zhang_2018_ICLR_mixup} & {SU} & 0.575 & 0.801 \\ 
+VAT\cite{Miyato_2018_PAMI_VAT}  & {SU} & 0.570 & 0.811 \\
% Random Bias & {} & 0.618 & 0.808 \\
% Adv Morph & {} & 0.541 & 0.798\\
+Adv Bias & {SU} & \textbf{0.650} & \textbf{0.826} \\
\midrule
+VAT\cite{Miyato_2018_PAMI_VAT} & SE  & 0.625 & 0.826\\
+Adv Bias & SE & 0.686 & \textbf{0.829}\\
\midrule
cGANs\cite{Chaitanya_2019_IPMI} & SE  & \textbf{0.710} & 0.823 \\
% Adv Bias\&Morph & {} & \textbf{0.716} & \textbf{0.825} \\% 
 \bottomrule
\end{tabular}

% \begin{tablenotes}
% \item Reported values are average Dice scores for the left ventricular myocardium segmentation under 20 test subjects. Results with highest scores in each category are represented by bold font.
% \end{tablenotes}
\end{threeparttable}
}
\end{table}



==> tables/random_aug.tex <==
\begin{table}[!ht]
\centering
\caption{\textbf{Segmentation accuracy of U-net trained with different \emph{random} data augmentation strategies in extremely low-data settings.} Reported values are average Dice scores for the left ventricular myocardium segmentation over 20 test subjects. Results with highest scores are represented by bold font.}
\label{tab:random}
\begin{tabular}{@{}lcccrr@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Spatial \\ Aug\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Morph \\ Aug\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Appearance\\ Aug\end{tabular}} & \multicolumn{2}{r}{\# Training subjects} \\ \cmidrule(l){5-6} 
 &  &  &  & 1 & 3 \\ \midrule
Plain &  &  &  & 0.293 & 0.544 \\
Affine & \yesmark &  &  & 0.467 & 0.779 \\
Affine+Intensity & \yesmark &  & \yesmark & 0.536 & 0.797 \\
Affine+Elastic & \yesmark & \yesmark &  & 0.439 & 0.799 \\
Affine+Bias & \yesmark &  & \yesmark & \textbf{0.618} & \textbf{0.808} \\ \bottomrule
\end{tabular}
\end{table}
